Tor circuit fingerprinting defenses using adaptive padding

Online anonymity and privacy has been based on confusing the adversary by creating indistinguishable network elements. Tor is the largest and most widely deployed anonymity system, designed against realistic modern adversaries. Recently, researchers have managed to fingerprint Tor's circuits -- and hence the type of underlying traffic -- simply by capturing and analyzing traffic traces. In this work, we study the circuit fingerprinting problem, isolating it from website fingerprinting, and revisit previous findings in this model, showing that accurate attacks are possible even when the application-layer traffic is identical. We then proceed to incrementally create defenses against circuit fingerprinting, using a generic adaptive padding framework for Tor based on WTF-PAD. We present a simple defense which delays a fraction of the traffic, as well as a more advanced one which can effectively hide onion service circuits with zero delays. We thoroughly evaluate both defenses, both analytically and experimentally, discovering new subtle fingerprints, but also showing the effectiveness of our defenses.

==> _none_.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> _region_.tex <==
\message{ !name(<none>.tex)}
\message{ !name(2-model.tex) !offset(-2) }
\section{Threat model}\label{sec:model}

\subsection{Tor Background??}

\subsection{Tor Threat Model}

One of the goals of Tor's threat model is to minimize the amount of metadata
that gets leaked to the various adversaries. While the Tor Project does not
have precise guidelines on the metadata that a LAN adversary or a relay
adversary can deduce from a user, it's clear that the more uncertainty provides
security for the users.

XXX

\subsection{Adversary Threat Model}

For the purposes of this research, we assume that the attacker is either a LAN
adversary or a relay adversary. This is because the attacker needs to be able
to extract fine-grained features out of the client's traffic and in particular
distinguish cells from each other. In this section we will go into more detail
on the various adversary classes.

\subsubsection{Relay adversary.}

An attacker can be part of the Tor network by setting up relays, and be able to
spectate or even influence the user's traffic. For this research, the main
adversary we are concerned about is guard adversaries, since they are in
position to know the location of the user and hence have more power if they
manage to carry out a circuit fingerprinting attack. A guard adversary can
easily perform traffic analysis attacks on the user's traffic since they have
full visibility on the Tor circuit and the cells transferred within. While they
cannot see the types of relay cells, they can still see the exact number of
incoming and outgoing cells.

\subsubsection{LAN adversary.}

A LAN adversary can be the network administrator of the user, their ISP, or any
other intruder between the user and their guard node. A LAN adversary can
collect TCP traces from the user, and then user heuristic algorithms to turn
those traces into fine-grained cell sequences. For the purposes of this
research we will assume this is indeed possible with high accuracy. The website
fingerprinting literature has been historically assuming that this is possible
with a high-probability of success, however in section \ref{section:lan} we
will analyze how that assumption ties into the circuit fingerprinting problem.

\subsection{Separating The Fingerprints}

The important message here is that we want to separate the circuit and website
fingerprinting problems. The reason is that WF is too easy for the adversary
and hard for us to defend against.  CF, on the other hand, is harder for the
adversary since the underlying traffic is the same and only the protocol
differs. Hence, we aim at answering the following questions.  First, how
effective can an adversary be in the harder CF problem? Second, can we provide
substantial defenses within Tor?

Separating website vs circuit fingerpriting
\begin{itemize}
\item reason1: separate problems, a lot of reaserch in WS-fingerprinting
\item reason2: more control over circuits: maybe easier to solve
\item light "criticism" to USENIX paper
\end{itemize}

\subsection{Scenarios}

\begin{outline}
\1 same content (site) and protocol (HTTP+TLS)
\1 EMPHASIS open world (harder for the adversary, but not much in our case)
\2 because the fingerprint is the protocol itself, not the content!
\1 singe-site (easier-for-adversary) vs multi-site
\end{outline}

\subsection{Experiment Methodology}

\begin{outline}
\0 Experimental methodology
\1 discuss selenium, traffic collection, modified tor client (show that it's a lot of work)
\1 discuss classifiers, features, etc
\end{outline}


\message{ !name(<none>.tex) !offset(-83) }


==> make.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> reviewers.tex <==
%%%%%%%%%%%%%%%%%%%%%%
% Revision response starts here
%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\onecolumn

\definecolor{blue(pigment)}{rgb}{0.2, 0.2, 0.6}
\newcommand\response[1]{{\color{blue(pigment)}#1}}

\section*{List of Major Revision changes}

In this letter we summarize the changes in our revision, and discuss how they address
the reviewers' comments.
For the reviewers' convenience, 
we attach at the end of this letter:
\begin{enumerate}
  \item A copy of the revised paper,
    so that section references link to the corresponding sections.
  \item A diff with the previous version.
\end{enumerate}



\section{Summary of Changes}
\label{rev:sumary_of_changes}

We would like to thank the reviewers for their insightful and relevant
comments. We believe that their comments have allowed us to significantly
strengthen our submission, making it more robust in terms of security and
easier to follow by readers.

\begin{enumerate}
  \item We restructured the paper, focusing first on the properties
  of \emph{onion handshakes} alone (\autoref{sec:design}), discussing how dummy handshakes can
  be generated, and then using these handshakes in different ways
  in our two defenses.

\item In the context of an isolated onion handshake, we performed a thorough timing analysis,
  we experimentally identified the distribution of fingerprintable timing features,
  we discuss ways to imitate them via padding machines,
  and we experimentally verify their effectiveness.

\item We significantly strengthened our delay-based strategy, realizing that a
  simple trick allows to improve performance without sacrificing privacy, by
  exploiting the base rate (previously we only considered the base rate in
  the analysis of the preemptive defense).  To reflect this change, we now call
  this defense ``fractional-delay'' (instead of ``high-latency'').

\item We provided bandwidth analysis of all suggested defenses.

\item We greatly improved the readability of our paper based on the insightful
  suggestions of all reviewers. We reduced the less important parts while expanding
  the main sections of the paper,
  simplified the paper structure and
  experiment flow, and we believe the final result is more streamlined and
  easier to follow.
\end{enumerate}

\section{Major Revision Criteria}

 \begin{enumerate}[label=(\Alph*)]

 \item \emph{Address timing in the two ways you propose in your response, but also the question about how $\lambda_u$ is chosen (in a way that is safe to expose to the middle node).}

   \response{
     The new section \autoref{sec:design} aims to provide a big part of the
     timing analysis that was missing from the paper. In this section:
     \begin{itemize}
      \item We study the timing characteristics of onion handshakes in isolation
        (the core part of circuit fingerprinting).
      \item We identify timing features that can act as fingerprints,
        both within the same circuit as well as between different circuits
        of the handshake.
      \item We experimentally identify the distributions of these features.
      \item We show that the timing can be appriximated by LogLogistic distributions,
      and experimentally verify that an adversary cannot distinguish real
      timing observations from fake ones.
      \item We discuss and provide detailed instructions on how to generate
      dummy handshakes (with proper timing characteristics) using padding machines.
     \end{itemize}

     We also added timing analysis discussions for both proposed defenses in
     sections \autoref{sec:fractional-delay} and \autoref{sec:pcp}.

     Concerning $\lambda_u$, we added a paragraph in \autoref{sec:evaluation-pcp}
     discussing the issue of leaking it to middle nodes and ways to prevent it.

     Note that the timing analysis in our paper remains preliminary:
     we believe that the analysis of a single handshake is the most important
     step in this direction, hence we studied it thoroughly in \autoref{sec:design}, including
     an experimental evaluation. On the other hand, we did not include timing in the experiments
     of sections \autoref{sec:fractional-delay}, \autoref{sec:pcp},
     leaving this as future work.
   }

 \item \emph{Analyze bandwidth overhead in the two ways you propose in your response, as well as emphasizing the tradeoff being made (lowering the bandwidth overhead affects what?  Security?  Latency (if no preemptive circuit is currently available, for example)?  How much?).}

   \response{ We added the bandwidth analysis that was missing from
     sections \autoref{sec:fractional-delay} and \autoref{sec:pcp}. We also
     added bandwidth information in figure \autoref{fig:experiment5_results}
     to highlight the tradeoffs involved.  }

 \item \emph{As you propose in your response, "implement and present the state machines needed to implement the PCP HSDir/Intro/RV padding, including the inter-cell timing distributions".}

   \response{ As part of the new section \autoref{sec:design}, we specified
     the state machine logic of our padding machines. We also show the code
     that implements it in our framework in \autoref{sec:padding-machines}.  }

 \item \emph{Analyze your defense against the best known attacks, which may include more features than you consider in this version.}

   \response{ With regards to non-timing features, we do provide the
     \emph{complete vector} of incoming/outgoing cells to the classifier. This
     is possible due to the fact that we work at the level of cells and onion
     sites have generally small sizes, fitting in a few hundred cells. Hence,
     any non-timing feature, eg percentages of incoming and outgoing packets
     (or any other feature from those from \cite{wf-tor}) is already included
     in the information provided by this vector.  We did try to explicitely
     include some of these features (number of incoming/outgoing packets) in
     the classification and it did not affect the results.
     
     We added discussion on this topic in \autoref{sec:vanilla-fpring}
    (where the feature vector is first introduced).

     With respect to timing features, we do use them in the experiments of
     \autoref{sec:design}, but not in those of \autoref{sec:fractional-delay}, \autoref{sec:pcp},
     as discussed in (B) above.
   }

 \item \emph{Clarify the description of PCP.}

   \response{ We believe that the addition of section \autoref{sec:design} and
     the overall structure simplification based on the reviewer's suggestions
     makes the entire paper clear and easier to follow.  }

\end{enumerate}

 \section{Individual Responses}

\vspace{20pt}

\response{ In addition to the list of expected major revisions above, we
  addressed most other comments and suggestions from the reviewers. In the
  section below we discuss some of the complex topics that occured and could
  benefit from discussion that could not fit in the paper. }

\vspace{20pt}

 \textbf{Reviewer~A}

 \begin{itemize}
 \item The middle node is used as the one to add the padding traffic, so the middle node learns the reality of the circuit.  Is that OK?  The middle node then doesn't learn the client IP, but does learn the client's guard, which seems at least a little bit bad?  (It's no worse than the current state of affairs, of course.)

 \response{
Doing the padding on the second hop has been a design decision to minimize the
padding traffic that travels inside the Tor network. In theory we could do
padding to the third hop, to reduce information leakage to the second hop, but
that would take padding traffic one hop further in. We thought that because the
information leakage to the middle is no worse than the current state of affairs
it was a reasonable tradeoff to take.
 }

\item If the guard is the adversary, it can tell the difference between RELAY and RELAY\_EARLY cells.  If you send a bunch of dummy cells before the circuit is extended to its final hop, won't that mess up the RELAY\_EARLY mechanism?

  \response{ This is a valid observation and one of the reasons that made
    practical implementation of PCP harder.  We believe that an alternative
    mechanism for restricting the number of hops on a Tor circuit is an
    interesting topic for future research, since the RELAY\_EARLY mechanism is
    restrictive and also leaks information.  We considered different ideas for
    improving the protocol but decided that it goes beyond the scope of the
    paper.

    A workaround that allows preemptive circuit padding in case of high levels
    of $\phi$ would be to have multiple preemptive circuits open, and send the
    fake handshakes on different circuits (opening new circuits as the number
    of RELAY\_EARLY gets exhausted), sending the application-layer data on the
    most recent fake/real rendezvous circuit.  We mention this workaround in
    \autoref{sec:pcp-evaluation} (also as a means to avoid leaking
    $\lambda_u$).  }

\item When injecting a traffic pattern into a circuit, where does the cell
that contains the padding instructions itself go?  Does it just act as
the first outgoing packet in the injected pattern?

\response{ Yes, exactly. }

\item In your Experiments 3 and 4 in Section 7, is a "positive" result an
indication that the classifier thought it was a \emph{real}
HSDir/introduction/rendezvous circuit, or a \emph{fake}
HSDir/introduction/padded-exit circuit?

\response { A positive result is an indication that the classifier thought it
  was a \emph{real} HSDir/introduction/rendezvous circuit. We clarified this in
  the tables in the appendix.}


\item In Figure 3, there's one EXTEND2 cell shown for the HSDir fetch and Introduction handshake, and none for the Rendezvous handshake.  What state is the circuit assumed to be in before seeing these patterns? Is it "extended to the middle node"?

  \response{ At that point the circuit has finished its preemptive phase and
    has been extended to \emph{Middle 2} as seen in
    \autoref{fig:intro-circuit-cell-flow}. Client rendezvous circuits do not
    extend past the \emph{Middle 2} since they use that second middle as the
    rendezvous point. On the other hand, introduction and rendezvous circuits
    have an extra extend round because they need to go to the right
    introduction point or HSDir node.
    }



\end{itemize}

 \textbf{Reviewer~B}

 \begin{itemize}
 \item Another general question: there's been a lot of attacks/defenses (mostly padding) in the WF landscape. I wonder if this work is just yet another padding defense. Especially, how will this work together with other WF defenses? This one focuses on defending (padding) against circuit fingerprinting, but there's still the WF. Will it be some sort of "double padding" if one wants to be secure? Is it practical? If it's not needed, then I'm missing some argument on why the PCP alone is sufficient.

 \response{
Our defenses only work at the Tor protocol layer and don't touch the
application layer at all. This means that they are compatible and combinable
with any other WF defenses that add padding or delays on the application
layer. Some sort of "double padding" might indeed be required if we are
interested in addressing both circuit fingerprinting and WF at the same time,
especially if the WF defense involves padding.
}

\item  Section 7 uses 10 sites for single-site, but I didn't find the information in section 8. Is it only one single-site, or the same as section 7 (which is 10 sites)? If the later, then what's the range of accuracy (in Figure 8), and why does the number of circuits differ so much in experiment 5 and 4 (in Appendix B)? If the former (one single-site), how will the result differ if more sites are evaluated? I think the answer probably needs a lot more evaluation than the current one (also, is 10 sites too few? Why not use more sites like in section 4?)

  \response{ The two experiments from sections \autoref{sec:experiment4}
    and \autoref{sec:pcp-evaluation} used the same number of single-site
    websites. We have clarified this in the latest version of the paper and in
    the appendix.

    The reason that the appendix numbers were different was because
    \autoref{fig:experiment5_results} uses results from just one single-site
    destination so that the figure looks as close as possible to the analytic
    evalution output. We felt that that focusing on a single site (and
    overlaying them on top of the analytic evaluation) to present our results
    was easier to understand. However, during the evaluation we performed the
    same procedure for all ten sites of the dataset and made sure that they all
    agree with the analytic evaluation.

    Ten sites might indeed seem few, but in single-site scenarios we opted for
    a smaller amount of destinations so that we can collect a greater number of
    circuits for each of them. Collecting traffic over Tor was a lengthy
    process since we used a slow fetch rate to avoid damaging the network, and
    we took steps between each fetch to ensure that each measurement is
    independent from the previous other.
}

\item Also, if I understand it correctly, from Figure 8, if $\phi=2$, then it
means if the user creates a new request every two seconds (on average), then a
dummy request should be sent every second (on average)? I understand that the
user "think time" is taken from a distribution in the evaluation, but in
reality, how can one know the rate of request by the user ahead of time so
enough dummy requests can be generated? The user may very well vary the rate (or
think time) between every request, so how can it be known in advance?

\response{The time between requests can indeed vary and this should not be a problem. What we
are interested in is the distribution of these times, which we can learn by
observing the user over some time period. An implementation, for instance, could
start with the fractional-delay defense, and if the system's usage increases
and low-latency is needed, it could switch to PCP using
the average rate of requests observed in the post recent period.
We added discussion on this point in \autoref{sec:pcp}.
}


\end{itemize}

 \textbf{Reviewer~C}

 \begin{itemize}
\item Ethics: You may or may not agree with Brian Levine's perspectives on Tor, But there is a strong case to be made that any paper on Onion Services, particularly defenses, should at minimum briefly point out that they are used in ways that are significantly harmful and that arguably outweigh their benefits. If you choose not to do so, I would like to know why.

  \response{ Thanks for the pointer to Brian Levine's research. We believe that
    Tor, as well as most other privacy/security tools -- like Signal and SSL,
    or even regular tools, like cars -- can see both positive and negative
    uses. We believe that Tor onion services specifically have enabled great
    positive use cases for society like whistleblowing platforms,
    metadata-resistant messaging and automated software update platforms. They
    are also actively used by organizations like The New York Times, BBC,
    Facebook and Deutsche Welle. We believe that onion services are still at
    the very early adoption stages, and as the technology gets more widely
    used, more positive use cases will float to the top.

    We also see the recent "encryption debate" about end-to-end encrypted
    messaging as a discussion with strong parallels to the topic of server-side
    anonymity:
    https://www.eff.org/deeplinks/2020/10/orders-top-eus-timetable-dismantling-end-end-encryption.

    Finally, we would like to point to the response of Tor's CEO to a more
    recent research paper about the same topic:
    https://arstechnica.com/gadgets/2020/11/does-tor-provide-more-benefit-or-harm-new-paper-says-it-depends/?comments=1
  }

\item Produce some data about the length of time that preemptive circuits live.
You would need this to set a value for lambda in any case. Data from real Tor
users would be better than data you produce locally, but a small case study
based on a reasonable range of behaviors might suffice. Note that I strongly
expect that some users will pause their use of Tor when a preemptive circuit is
open, leading to very long delays in some cases. It's important to capture and
understand this case when figuring out the distribution.

\response{ A user study would certainly be interesting, but due to time
  constraints we had to focus on the requested major revisions.

  Concerning idle periods, it is true that  preemptive circuits can live for a
  long time. In these cases it might be preferable to apply heuristics that
  switch back to the fractional-delay defense. We added a discussion on this topic
  in \autoref{sec:pcp}.
  }

\item 1. a. Consider an alternative distribution like Pareto instead of exponential. This is likely to provide a much closer fit to real user data.

  \response{
    Another good suggestion, we added a footnote about this possibility.
    It would however require to adapt our analytic evaluation,
    which should be doable, although space-consuming.
    Moreover due to time constraints we had to prioritize the timing-related revisions.
  }

% \item 3. Consider providing a diagram of some of the cases that can occur in the security analysis.
% - No dummy triplets, no connection
% - No dummy triplet, connection
% - 1+ dummy triplet, no connection
% - 1+ dummy triplet, connection

% \response{XXX}


\item Why SVM and DT classifiers and not others?

  \response{ Our research project originally started with the idea of applying
    deep learning to the circuit fingerprinting space similar to
    \cite{deepfingerprinting}.  However, we found that basic ML classifiers
    like SVM and DT had the same accuracy results as neural networks for our
    positive offensive results. Furthermore, it was easier understanding the
    fingerprints of DT classifiers when it came to results like the esoteric
    fingerprints found in \autoref{sec:evaluation-delay}. Based on these
    observations we decided to use the simpler SMT and DT classifiers for this
    work. We also added a note about this choice in \autoref{sec:methodology}.  }
\end{itemize}

 \textbf{Reviewer D}

 \begin{itemize}
 \item It is not clear to me that ML is the right tool for this endeavor.  It seems to me that the ML techniques used in this work simply confirm what a close reading of the construction would already tell the reader (with the exception of the results in Table 3 that highlight an interesting issue).  This problem is exacerbated by the lack of timing information in the classifier -- the features that are fed into the ML algorithms feel like they could be examined manually, which would be more clear and convincing.

   \response{ It is true that some of the early experiments could have been
     confirmed just by close reading of the cell sequence. We opted for using ML
     there too, because that was also the approach that Kwon et al. took. Based
     on this recommendation, in this latest revision of the paper we greatly
     simplified the sections of those early simple experiments and instead put
     focus on the more interesting final classifications experiments. }

 \end{itemize}

 \textbf{Reviewer E}

 \begin{itemize}

 \item I am feeling uneasy about the formalization you present in Section 3.3. Indeed, you mention some of my concerns in the discussion section. I don't believe the stated formalization captures many commonly considered adversary assumptions. For example, as you note, this adversary is performing classifications per connection. In practice, a network adversary could make circuit classifications using a client's history of circuit behavior. An adversary is often assumed to have multiple vantage points in the network (for example, controlling multiple relays or the destination service); I do not think this is captured by your formalization. An active adversary may be able to influence connections by withholding certain packets and observing timeout behaviors, for instance, but I don't think this is captured either. Also, I don't believe the notion of "trace" is defined, but it is important to precisely define what information the adversary is given.

   \response{
     We agree that the adversary game was too immature to belong in the final
     version of the paper. We thought it would inspire further research but in
     the end it just brought confusion. We decided to remove it and use the
     space to highlight the need for further formalization in the discussion
     section.  }


   \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%
% Revision response ends here
%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "make"
%%% End:

